RAFCON: a Graphical Tool for Task Programming and Mission Control

There are many application fields for robotic systems including service robotics, search and rescue missions, industry and space robotics. As the scenarios in these areas grow more and more complex, there is a high demand for powerful tools to efficiently program heterogeneous robotic systems. Therefore, we created RAFCON, a graphical tool to develop robotic tasks and to be used for mission control by remotely monitoring the execution of the tasks. To define the tasks, we use state machines which support hierarchies and concurrency. Together with a library concept, even complex scenarios can be handled gracefully. RAFCON supports sophisticated debugging functionality and tightly integrates error handling and recovery mechanisms. A GUI with a powerful state machine editor makes intuitive, visual programming and fast prototyping possible. We demonstrated the capabilities of our tool in the SpaceBotCamp national robotic competition, in which our mobile robot solved all exploration and assembly challenges fully autonomously. It is therefore also a promising tool for various RoboCup leagues.

==> features.tex <==
Not all of the features of RAFCON have been described, yet. While it is not possible to mention all in the scope of this paper, at least the most important remaining ones shall be listed here.

% storage format
RAFCON stores state machines in a human readable file format. Each state is stored in its own folder on the file system, containing separate JSON files for core and GUI data. The folder structure directly reflects the state machine tree. This enables versioning of state machines in repositories and thus collaborative state machine programming.

% state machine generation
The comprehensive core API allows for programmatic state machine generation from within another tool, e.\,g. task planners like CRAM.



==> related_work.tex <==
%RAFCON falls in a broad category, which can be named \textit{robot programming}. This field is huge and includes \textit{Programming by Demonstration} utilizing \textit{teleoperation}, \textit{kinesthetic teaching} or \textit{observational learning} \cite{billard2008robot}. Using these methods, a robot can be taught arbitrary motions. However, definitions how to react on certain inputs, like camera images, or external events are very limited.

%Another approach are the aforementioned \textit{symbolic task planners}, for which CRAM \cite{beetz2010cram} is an example. In theory, those systems accept natural high-level commands such as ''set the table for breakfast`` and then plan the involved steps using a reasoning and prediction system with the help of detailed models and world knowledge. This is a top-down approach, contrasting the bottom-up approach of hierarchical state machines.

%\textit{Finite state machines} (FSM, or extensions of them) are heavily used for programming complex software or representing extensive robot behaviors \cite{bohren2011towards, jentzsch2013tums, nguyen2013ros}. Complex decision trees would otherwise be very tedious to describe in huge switch and if-else cascades (``spaghetti code''). A well known kind of state machine is the \textit{deterministic finite state machine} (DFA)~\cite{krithivasan2014theory}. As state machines do not produce any output, the \textit{finite state transducer} (FST) augments the DFA with an output alphabet and an output function \cite{krithivasan2014theory}.

%Another extension of FSM is \textit{statechart}, originally invented by Harel~\cite{harel1987statecharts}. Some of the concepts introduced by Harel are orthogonality (which is equal to concurrency), hierarchy and a special form of broadcast communication.

%A further statechart dialect is \textit{SyncCharts}~\cite{andre1995synccharts}. It also includes concurrency, hierarchy and information exchange concepts, yet in addition offering enhanced preemption capabilities and support for transition priorities. The clear focus of SyncCharts lies on \textit{reactive systems}, i.\,e. systems reacting to external events. The fact that there exists an exact formal notation for SyncCharts is a clear advantage over statecharts.

%\textit{Flowcharts} are another type of diagram for modeling behaviors or processes. The graphical representation of state diagrams like statechart and SyncCharts share some similarities with flowcharts. Yet, the formalisms heavily differ. One distinction is the way in which a transitions is determined. State diagrams are event-driven, i.\,e. events trigger their corresponding transitions. For flowcharts, transitions are either automatically chosen (if there is only one) or depend on the outcome of a state~\cite{simons2000compositional}. Strictly speaking, flowcharts are no state machines, however we include these charts in our broader sense of state machines.

%For RAFCON, we deliberatively decided against an event-driven design. State diagrams may have advantages in reactive systems in which events are in the foreground, such as  stopwatches~\cite{harel1987statecharts} or watchdogs for sensor monitoring~\cite{andre1995synccharts}. However, with increasing complexity, event-driven system are error-prone~\cite{parent2006possible}, resulting from complex topics that need to be tackled, like event caching and priorization, event expiration and parallel event handling~\cite{lamport1978time}. Therefore, RAFCON is inspired more by flowcharts, letting states decide about the next transition to follow. Nevertheless, this decision can be based on events, if the state registered a callback.

%In our opinion, statecharts and SyncCharts offer too many arguable features and concepts. For example, they allow transitions to cross hierarchy boundaries, which is contrary to important software engineering principles like encapsulation and composability~\cite{maier2010deprecating}. There are many more concepts (transition guards, transition hooks, deferred events, \ldots). All of these can unburden the programmer from some work, while at the same time increasing complexity and with this error-proneness of the underlying system. Therefore, the RAFCON core (see Section~\ref{sec:core_framework}) is kept slim, with only an essential feature set.

%All state machine types mentioned so far are general concepts that are not bound to robotic applications. There exist also many solutions clearly invented for robotic purposes. In~\cite{thomas2013new}, robots are programmed using generic action components which are mapped to statecharts. Another state machine like system for representing robot tasks are skill nets~\cite{thomas2003Error}. However, their range of application is rather limited, as they lack concepts for hierarchy, concurrency and explicit data handling.

%A proper tool for programming complex robotic tasks must not only have concepts for hierarchies and concurrencies but also needs a GUI intuitively integrating these concepts and allowing for efficient programming. There is a huge number of visual programming tools for a variety of different domains\footnote{See http://blog.interfacevision.com/design/design-visual-progarmming-languages-snapshots/ for a graphical overview}. Worth mentioning is for example \textit{Scratch}, which is intended for education and allows for both imperative and event-driven programming~\cite{resnick2009scratch}. The idea of using a visual state machine concept for programming robots is not new, either. One famous example for programming LEGO Mindstorms robots is \mbox{\textit{NXT-G}}~\cite{kelly2010lego}. There are also a lot of hardware-independent tools, however all of them suffer some kind of problem. Some are no longer maintained, like \textit{ROS Commander} \cite{nguyen2013ros}, \textit{RobotFlow} \cite{cote2004code} or \textit{MissionLab}~\cite{arkin2006missionlab}, others are closed source/commercial, such as \textit{Gostai Studio}~\cite{baillie2008urbi}, or lack a graphical editor, for example \textit{SMACH}~\cite{bohren2010smach}.

%Further state machine libraries that do not have a graphical user interface (GUI) at all are also existing, such as~\textit{Boost statechart} \cite{doenni2007boost} or \textit{Spring Statemachine}~\cite{pivotalsoftware2016spring}.

%While all of the mentioned tools were not considered as sufficient for our needs, we adopted many or their features for RAFCON. SMACH for example has a similar concept of outcomes and data ports, called input/output keys. \mbox{NXT-G} visualizes its input and output data ports as well as the data flows, just as RAFCON. ROS Commander includes a graphical editor, however it only offers a limited number of features.
%
%In our opinion, a GUI with a graphical representation of the state machine and the option of editing, is an important supportive feature of a programming tool for robots. However, this is not an easy feature to achieve, as bigger state machine with deep hierarchies tend to become very complex. Most visual programming tools do not support hierarchies, like \mbox{NXT-G}, or show elements on different hierarchy levels in the same size, such as SMACH, which does not scale.
%
%The graphical representation of RAFCON is inspired by the flow control tool \textit{Bubbles}, which has been developed at our institute some years ago~\cite{widmoser2012interaction}. This tool was internally used with success, yet it had many limitations. This is why RAFCON was created, completely from scratch, but with ideas from Bubbles and a long list of requirements identified by roboticists of different areas. 

==> state_machine_definition.tex <==
The concepts of a RAFCON state machine, described in the previous section, contain components distinguishing it from all other state machines mentioned in Section~\ref{sec:related_work}. Therefore, in the following, we will give a formal notation of our state machine using predicate logic and set theory.

Concerning the execution semantics, the RAFCON state machine model resembles a FST with the Moore model~\cite{krithivasan2014theory}, as the actions of the state machine take place during the execution of a state and not during the transition.
%Furthermore only execution states perform actions. The results of those actions are mapped to discrete outcomes.

However, relating to data handling, our state machine approach is similar to the Mealy model~\cite{krithivasan2014theory}. The main difference to the Mealy model is that the input for a state is not associated with the transitions but is passed via dedicated data edges, called data flows. More specifically, states forward their output as input to other states (1$\times$n relation).

First, we define the elements of a state machine and its relationships. Then, the definition of a RAFCON state machine is provided.

\begin{figure}[!htb] %[H]
	\centering
	\includegraphics[width=0.5\columnwidth]{state_machine_tree.pdf}
	\caption{The hierarchical state machines in RAFCON can be represented as a tree. The root state, all direct children of a hierarchy state (HS), as well as each direct child of a concurrency state (CS) can be considered as a separate, flat state machine (dashed rectangles). The leaves of the tree are typically execution states (ES), but could also be empty hierarchy or concurrency states.}
	\label{fig:state_machine_tree}
	%\vspace{-1em}
\end{figure}

\begin{mydef}[State]
	\label{def:state}
	A state $s$ is an entity having an execution mode and type: $\sem(s) \in \{\textrm{active, inactive}\}$, $\type(s) \in \{\textrm{execution, hierarchy, concurrency}\}$. The different states are called \textit{execution states}, \textit{hierarchy states} and \textit{concurrency states}, respectively.
\end{mydef}

\begin{mydef}[RAFCON state machine tree (RST)]
	\label{def:statemachine_tree}
	A \mbox{RAFCON} state machine tree (RST) is a \textit{rooted tree} $G = (S, E)$ with $r \in S$ being the \textit{root vertex}. $S$ is the set of nodes and $E$ is the set of edges which define the \textit{tree-order} $x < y$ ($\forall x \in V \setminus r: r < x$), following the definition of~\cite[p. 13--15]{diestel2005graph}. All vertices $s \in S$ are states, therefore $r$ is also titled the \textit{root state}. All states $s \in S$ with $\type(s) = \textrm{execution}$ must be \textit{leaves} of the tree. In Fig.~\ref{fig:state_machine_tree}, an example of a \mbox{RAFCON} state machine tree is shown.
\end{mydef}

% Old state machine graph definition
%\begin{mydef}
%A RAFCON state machine graph (RSG) consists of a directed hypergraph DH = $(N,E)$ where $N$ is the set of nodes and $E$ is the set of edges
%%(S) corresponds to the set of states and the set of directed edges (T, hyperarcs) corresponds to the set of the transitions
%(for a formal definition of hypergraphs and hyperarcs/hyperedges used here see \cite{bernardo2009formal}). The nodes of the graph are a strictly partially ordered set, that is ordered by the transitively reduced binary relation $parent(a,b)$ (covering relation) (see \cite{davey2002introduction}), where $a \in S$ and $b \in S$. Only one state (the root state) is not preceded by another state through the $parent()$ relation. For the set of nodes M of a hyperarc holds: $\forall m \in M: (\exists m^\prime \in M: \exists p \in S: parent(p, m) \land parent(p, m^\prime) \land \neg (\exists m^{\prime\prime} \in M: \exists p^{\prime\prime} \in S: parent(p^{\prime\prime}, m^{\prime\prime}) \land \neg (p = p^{\prime\prime}))) \lor (\exists p \in S: parent(p,m) \land p \in M)$.
%\label{definition:statemachine_graph}
%\end{mydef}

%\begin{figure}[!htb]
%\minipage{0.24\textwidth}
%  \includegraphics[scale=0.15]{./hypergraph.pdf}
%  \caption{Hypergraph}
%  \label{fig:hypergraph}
%\endminipage
%\minipage{0.24\textwidth}
%  \includegraphics[scale=0.15]{./hyperarchs.pdf}
%  \caption{Hypergraph with hyperarcs}
%  \label{fig:hyperarchs}
%\endminipage
%\end{figure}

%A example state machine graph is shown in figure \ref{fig:hierarchy_state}.

%\begin{figure}
%\begin{center}
%  \includegraphics[scale=0.3]{./hierarchy_state.pdf}
%  \caption{Nested hierarchy state with data flow visualization}
%  \label{fig:hierarchy_state}
%\end{center}
%\end{figure}

% \begin{figure}
% \begin{center}
%   \includegraphics[scale=0.3]{./concurrency_state.pdf}
%   \caption{Concurrency state with data flow visualization}
%   \label{fig:concurrency_state}
% \end{center}
% \end{figure}

Using the tree-order of a RST, we can define further relations on such a tree:

\begin{mydef}[parent]
	\label{def:parent}
	In a RST $G = (S, E)$, state $p \in S$  is called a parent of state $s \in S$, if $p < s$ and $p$ and $s$ being \textit{neighbors}~\cite[p. 3]{diestel2005graph} (i.\,e. share a common edge $e \in E$). This is written as $\parent(p, s)$.
\end{mydef}

\begin{mydef}[children]
	\label{def:children}
	In a RST $G = (S, E)$, the children of a state $p \in S$, written as $\children(p)$, is defined as the set of all $s \in S: \parent(p, s)$.
%	$\parent(p, s) \Rightarrow \child(s, p)$; thus it is the inverse of the parent relation (literally s is called ''child of p``);
% $children(p)$ is the set of all states where $parent(p, s)$ holds.
\end{mydef}

\begin{mydef}[siblings]
	\label{def:sibling}
	In a RST $G = (S, E)$, two states $s, s' \in S$ are said to be siblings, write $\siblings(s, s')$, if $\exists p \in S: \parent(p, s) \land \parent(p, s')$. Note that $s$ and $s'$ can be the same state.
%$\siblings(s, s')$ is true if $\exists p \in S: \parent(p, s) \land \parent(p, s')$ (literally s and $s'$ are siblings)
\end{mydef}

%\begin{mydef}[hierarchy]
%	\label{def:hierarchy}
%	In a RST $G = (S, E)$ with $p \in S$: $\hierarchy(p) \coloneqq \children(p) \cup p$
%\end{mydef}

%\begin{mydef}[Hierarchical Closure]
%A set of states $X \subseteq S$ is said to be closed under the parent relation if for all $x \in X$: $x \in S \land \exists p \in S: \parent(x, p) \land (\sem(x) = \textrm{active}) => (\sem(p) = \textrm{active})$. This means that in a hierarchical closed graph a state with children is always active if one child is active.
%\label{def:hierarchical_closure}
%\end{mydef}

The following definitions~\ref{def:logical_port} and~\ref{def:transition} are related to the logical flow of a RAFCON state machine.

\begin{mydef}[Logical port]
	\label{def:logical_port}
	A logical port is a couple $l = (s, t)$ with state $s$ and type $t \in \{\textrm{income, outcome}\}$, $\textrm{outcome} \in \{\textrm{aborted, preempted, common}\}$. A logical port with any type of outcome is literally called an \textit{outcome}.
\end{mydef}

\begin{mydef}[Transition]
	\label{def:transition}
	A transition is a couple $t = (l_1, l_2)$ with $l_1 = (s_1, \textrm{outcome})$, $l_2 = (s_2, \textrm{income})$ both being logical ports and $\siblings(s_1, s_2)$. $l_1$ is called the \textit{source port}, $l_2$ the \textit{target port}.
\end{mydef}

The following definitions~\ref{def:data_port} through~\ref{def:value_vector} are related to the data handling of a RAFCON state machine.

\begin{mydef}[Data port]
	\label{def:data_port}
	A data port is a triple $d = (s, t, v)$ with state $s$, type $t \in \{\textrm{input, output}\}$ and default value $v \in A$, whereat $A$ is an arbitrary alphabet.
\end{mydef}

\begin{mydef}[Data flow]
	\label{def:data_flow}
	A data flow is a couple $F = (d_1, d_2)$ with $d_1 = (s_1, t_1, v_1)$ and $d_2 = (s_2, t_2, v_2)$ both being data ports, which must fulfill

	\begin{math}\begin{array}{lc}
		(\siblings(s_1, s_2) \land t_1 = \textrm{output} \land t_2 = \textrm{input}) & \lor  \\
		(\parent(s_1, s_2) \land t_1 = t_2 = \textrm{input}) & \lor  \\
		(\parent(s_2, s_1) \land t_1 = t_2 = \textrm{output}) &
	\end{array}\end{math}
	
	Thus, a data flow exists either between two sibling states or between a child and its parent state.
\end{mydef}

\begin{mydef}[Data port value]
	\label{def:data_port_value}
Each data port $d = (s, t, v)$ has a value $a$ of a certain alphabet $A$: $\val(d) = a$. By default, $\val(d) = v$. If $t = \textrm{output}$ and $\type(s) = \textrm{execution}$, then the output function $\mu_e$ can determine this value (see Definition~\ref{mydef:statemachine}). If there is a data flow $f = (d', d)$, then the value of the source port $d'$ defines the value of the target port $d$: $(\val(d') = a') \Rightarrow (\val(d) = a')$.
\end{mydef}

\begin{mydef}[Value vector]
	\label{def:value_vector}
	A value vector $V_{s', t'}$ with state $s'$ and data port type $t' \in \{\textrm{input, output}\}$ is a vector consisting of all values assigned to all ports of that type at that state, thus $[\val(d_1), \val(d_2), \ldots]$ for all $d_i = (s=s', t=t', v_i)$.
\end{mydef}

With the definitions of the elements of a state machine and its relations, the state machine definition can be given:

\begin{mydef}[HFPD]
A \textit{hierarchical, parallel, finite state machine with data flows} (HPFD) is a 11-tuple $(\Sigma,W,G,L,T,D,F,M,S_\text{exit},T_\text{exit},P)$, where

\begin{itemize}
	\item $\Sigma$ is the data alphabet. This is typically $\mathbb{R}$, but can also contain e.\,g. strings or lists.
 
	\item $W(\tau): \tau \mapsto \Sigma^n, n \in \mathbb{N}$ is a vector function representing the world state at time instance $\tau$. This vector function serves as access to global variables, see Section~\ref{sec:core_framework}, or sensor readings. In robotic contexts, $\Sigma$ is not finite and thus neither are the elements of $W(\tau)$.
	
	\item $G = (S, E)$ is a RST, with the set of states $S$ being finite and non-empty.
	
	\item L is the set of logical ports, whereat $\forall s \in S:(\exists! l \in L: l = (s, \textrm{income})) \land (\exists! l' \in L: l'=(s, \textrm{aborted})) \land (\exists! l'': l'' = (s, \textrm{preempted}))$. Thus, all states must have exactly one logical of each type income, aborted and preempted. Furthermore, $\forall l = (s, t) \in L: s \in S$.
	
	\item $T$ is the set of transitions, with $\forall t = (l_1, l_2) \in T: l_1 \in L \land l_2 \in L$.
	
	\item $D$ is the set of data ports, with $\forall d = (s,t,v) \in D: s\in S \land v \in \Sigma$.
	
	\item $F$ is the set of data flows, with $\forall f = (d_1, d_2) \in F: d_1, d_2 \in D$.
	
	\item $M$ is the set of all output functions $\mu_e: V_{e, \textrm{input}} \times W(\tau) \mapsto L_{e, \textrm{outcome}} \times V_{e, \textrm{output}}$ for the execution states $e \in S$. Here, $V_{e, \textrm{input}}$ and $V_{e, \textrm{output}}$ are the input respectively output value vectors of $e$ and $L_{e, \textrm{outcome}}$ being the set of all logical ports $l = (s = e, t = \textrm{outcome}) \in L$. The output functions have access to the current world state $W(\tau)$. Together with the input port values, they determine the outcome port and the values assigned to the output ports. The evaluation of an output function takes a certain amount of time $\Delta \tau > 0$.
	
	\item $S_\textrm{entry} \subset S$ is the set of all \textit{start states}. A start state is the state evaluated first when entering a hierarchy state. Thus, for each hierarchy state $h \in S$, there is at most one state $s \in S_\textrm{entry}$ with $\parent(h, s)$.
	
	\item $T_\textrm{exit}$ is a set of couples $t_\textrm{exit} = (l_1, l_2)$ with $l_1 = (s_1, t_1 = \textrm{outcome}) \in L$ being the source outcome, $l_2 = (s_2, t_2 = \textrm{outcome}) \in L$ being the target outcome and $\parent(s_2, s_1)$. If the execution (see further down) reaches an outcome being the source port of a couple $t_\textrm{exit} \in T_\textrm{exit}$, then the state $s_2$ of the target outcome is left at this target outcome $l_2$.
	
	% \item $\nu_h: h \mapsto children(h)$ is the set of all entry functions of all hierarchy states $h$
	% 
	% \item $\xi_h: MO \mapsto hierarchy(h)$ is the set of all outcome transitions functions of all hierarchy states $h$, where $\forall \{m, o\} \in MO: m \in children(c) \land o \in O \land parent(o) = m$
	% 
	% \item $\varpi_c: c \mapsto children(c)$ is the set of all entry transition functions for all concurrency states $c$
	
	\item $P$ is the set of all outcome functions $\rho_c: \mathbb{P}(L_{\children(c)\textrm{, outcome}}) \mapsto L_{c, \textrm{outcome}}$ for the concurrency  states $c \in S$. Here, $\mathbb{P}(L_{\children(c)\textrm{, outcome}})$ is the power set of all outcomes of all $\children(c)$ and $L_{c, \textrm{outcome}}$ is the set of all logical ports $l = (s = c, t = \textrm{outcome}) \in L$. If one child state of $c$ exits ($c$ being a \textit{preemptive concurrency state}) or all children of $c$ have exited ($c$ being a \textit{barrier concurrency state}), then $\rho_c$ determines the outcome of $c$ on which $c$ is exited.
	
	%\item $\rho_c: P(MO) \mapsto CO$ is the set of all outcome transition functions of all concurrency states $c$, where $\forall \{m, l\} \in MO, \forall co \in CO: m \in children(c) \land l \in L \land l = (m, outcome) \land co \in L \land co = (c, outcome)$. $\rho_c$ defines the outcome of the execution of concurrency states and ultimately decides when its execution is finished.
\end{itemize}

The following properties apply for HPFDs:

\begin{itemize}	
	\item If a hierarchy state is executed, then the execution directly starts with the entry state defined by $S_\textrm{entry}$ and finishes when an exit outcome defined by $T_\textrm{exit}$ is reached.
	
	\item If a concurrency state is entered, all of its children are entered in parallel. Thus, the execution splits up. The outcome function $\rho_c$ defines on which outcome to leave the concurrency state.
	
	\item Initially, all states are inactive: $\forall s \in S$, $\sem(s) = \textrm{inactive}$. When a state $s$ is entered, meaning that the execution reaches an income $l = (s, \textrm{income}) \in L$, then $\sem(s) = \textrm{active}$. Accordingly, when a state is left, meaning that the execution reaches an outcome $l = (s, \textrm{outcome}) \in L$, then $\sem(s) = \textrm{inactive}$.
	
	\item Every port $l = (s, t = \textrm{outcome}) \in L$ can only be the source of either one $t \in T$ or one $t_\textrm{exit} \in T_\textrm{exit}$.
	
	\item Transitions are only allowed in hierarchy states.
\end{itemize}
\label{mydef:statemachine}
\end{mydef}

With these definitions, for example deadlock detection and reachability analysis are possible in future work. Furthermore, it enables comparisons with other state machine approaches.
%In order to achieve that an extension to this definition will be given, that allows to represent a HPFD completely as a graph. A hypergraph as defined by Bernardo et al.~\cite{bernardo2009formal} turned out to be a promising approach.

%As we are currently working on a useful formal definition of a world model we just give a very abstract model of it in definition~\ref{mydef:statemachine} to just be a vector of symbols of a given alphabet. In fact the world model holds all information the robot has about its environment, which are continuously updated by sensor readings.

%% Explanation of old transition functions
%A short explanation of all transition functions is given now. $\mu$ basically defines the execution of an execution state. Optionally based on input forwarded by data flows, the state generates output, which can be forwarded to other states, and returns an outcome. $\xi$ defines the successor state in a hierarchy based on the executed child state and its outcome. $\varpi$ defines the entry states of a concurrency state. Finally, $\rho$ defines the successor definition of concurrency states and decides when its execution is finished. 
%There exist two subtypes of the concurrency state type: the preemption concurrency state and the barrier concurrency state. The barrier concurrency state waits for all its children to finish and then transits to its following state. In the preemption concurrency state the first child, that finishes its execution, preempts all its siblings.
% The barrier concurrency state waits for all its child states to finish and only then transits to the next state. A dedicated decider state returns a specific outcome and specific output depending on the output of all child states. This decider state terminology is only relevant for programming purposes and is implicitly encoded into the above outcome transition function.
% Notice that there is no separate data forward function for the concurrency states as there are no transitions between siblings and thus the data is associated with the transitions.
